SoK: Differential Privacy on Graph-Structured Data

In this work, we study the applications of differential privacy (DP) in the context of graph-structured data. We discuss the formulations of DP applicable to the publication of graphs and their associated statistics as well as machine learning on graph-based data, including graph neural networks (GNNs). The formulation of DP in the context of graph-structured data is difficult, as individual data points are interconnected (often non-linearly or sparsely). This connectivity complicates the computation of individual privacy loss in differentially private learning. The problem is exacerbated by an absence of a single, well-established formulation of DP in graph settings. This issue extends to the domain of GNNs, rendering private machine learning on graph-structured data a challenging task. A lack of prior systematisation work motivated us to study graph-based learning from a privacy perspective. In this work, we systematise different formulations of DP on graphs, discuss challenges and promising applications, including the GNN domain. We compare and separate works into graph analysis tasks and graph learning tasks with GNNs. Finally, we conclude our work with a discussion of open questions and potential directions for further research in this area.

==> ArXiv SoK DP on Graph-Strucutred Data(1)/summary_table.tex <==
% \begin{table*}[h!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccccl}
% % \toprule
% Reference & GNN & Edge-DP & Node-DP & Year & Context \\ \midrule
% Nissim et al. \cite{nissim2007smooth} &                                   & \checkmark                             &  \checkmark                            &   2007    &         Private estimation for a spanning tree of a graph               \\
% Hay et al. \cite{hay2009accurate} &                                   &       \checkmark          &                      &    2009     &       Private graph degree estimation               \\
% Mir et al. \cite{mir2009differentially} &                                   &     \checkmark                        &                             &      2009    &      Private graph estimation               \\
% Gehrke et al. \cite{gehrke2011towards} &                                  &                               & \checkmark                             &  2011 & Zero-knowledge graph statistics estimation                             \\
% Machanavajjhala et al. \cite{machanavajjhala2011personalized} &                                  & \checkmark                               &                        &  2011    &  Privacy in social graphs                             \\
% Sala et al. \cite{sala2011sharing} &                                  & \checkmark                              &                     &    2011     &  Release of private graphs                             \\
% Karwa et al. \cite{privateAnalysisGraph} &                                   & \checkmark                              &                     &     2011   &            Private subgraph counting                   \\
% Gupta et al. \cite{gupta2012iterative} &  & \checkmark & & & Synthetic data for graph cuts
% \\
% Karwa et al. \cite{karwa2012differentially} &                                   & \checkmark                               &                      &  2012    & Release of graph degree sequences \\
% Mir et al. \cite{mir2012differentially} &                                   &         \checkmark                       &                             &  2012    &      Private release of graph distribution \\

% Blocki et al. \cite{blocki2013differentially} &                                  &         \checkmark       & \checkmark                             &  2013  &    Restricted sensitivity for DP                        \\
% Chen et al. \cite{chen2013recursive} &                                   &                              & \checkmark                              &   2013    &      Private graph database aggregation                  \\
% Kasiviswanathan et al. \cite{kasiviswanathan2013analyzing} &                                   &                              &  \checkmark                            &      2013    &      Private graph analysis               \\
% Shen et al.* \cite{shen2013mining} &                                   &                              &                               &   2013     &     Private graph pattern mining                  \\
% Wang et al. \cite{wang2013differential} &                                   &        \checkmark                      &                               &       &      Private spectral graph analysis                  \\
% Wang et al. \cite{wang2013preserving} &                                   &        \checkmark                      &                               &        &     Private spectral graph analysis                  \\
% Chen et al. \cite{chen2014correlated} &                                   &         \checkmark                     &                               &     2014    &    Correlated network data release                  \\
% Lu et al. \cite{lu2014exponential} &                                   & \checkmark                             &                              &     2014      &       Private estimation of graph model parameters             \\
% Task et al. \cite{task2014should} &                                   & \checkmark                              & \checkmark                             & 2014   &    Private social network analysis \\

% Day et al. \cite{day2016publishing} &                                   &                              & \checkmark                   &           2016        &     Private graph distribution release        \\
% Jorgensen et al. \cite{jorgensen2016publishing} &                                   & \checkmark                              &                        &   2016   & Private attributed graph models \\
% Raskhodnikova et al. \cite{raskhodnikova2016lipschitz} &                                   &            & \checkmark                &     2016         &  Private release of graph statistics                             \\
% Wang et al. \cite{wang2016using} &                                   & \checkmark                              &                               &          &        Private aggregation of data             \\
% Qin et al. \cite{qin2017generating} &         &                 \checkmark              & \checkmark                             &   2017   &        Private release of social graphs                 \\
% Zhu et al. \cite{zhu2017differential} &                                   & \checkmark                              & \checkmark                       &       &   Applications of differential privacy \\
% Cormode et al. \cite{cormode2018privacy} &                                   & \checkmark                              & \checkmark                       &    2018   & Private data release                              \\
% Macwan et al. \cite{macwan2018node} &                                   &                              & \checkmark                         &  2018   & Private release of graph data                 \\

% Arora et al. \cite{arora2019differentially} &                                 & \checkmark                               &                     &    2019     & Graph sparsification \\
% Yuxuan et al. \cite{yuxuan2019graph} &                                   &                              & \checkmark                              &       &      Private histogram release                  \\

% Liu et al. \cite{liu2020publishing} &                                   &                              & \checkmark                              &   2020   &       Node strength distribution                  \\
% Sajadmanesh et al.** \cite{sajadmanesh2020locally} &  \checkmark                                 &                               &                  &    2020        &  Private, model-agnostic framework for GNNs                             \\
% Zhang et al. \cite{zhang2020community} &                                   &                              & \checkmark                              &    2020   &      Private social graph release                  \\
% Zhang et al. \cite{zhang2020differentially} & & & \checkmark & & Control-flow graph coverage analysis \\
% Iftikhar et al. \cite{iftikhar2021dk} &                                   &                              & \checkmark                        &      & Private release of degree distribution               \\
% Fichtenberger et al. \cite{fichtenberger2021differentially} & & & \checkmark & 2021 & Private dynamic graph algorithms \\ 
% Igamberdiev et al.** \cite{igamberdiev2021privacy} & \checkmark                                   &                                &   &    & Private text classification \\
% Imola et al. \cite{imola2021locally} &                                  & \checkmark                               &                       &    2021  &     Private sub-graph counting                          \\
% Lan et al. \cite{lan2021sensitivity} &                                   &                              & \checkmark                              &   2021     &     Private node strength histogram release                  \\
% Liu et al. \cite{liu2021graph}                               &                                   &                              &  \checkmark & 2021 &  Private degree histogram release \\
% Olatunji et al.** \cite{olatunji2021releasing} & \checkmark                                  &                              &                              & 2021 &   Private GNN and graph data release \\
% Sealfon et al. \cite{sealfon2021efficiently} &                                   &                              & \checkmark                              &  2021 &    Private graph density estimation                        \\
% Zhang et al.** \cite{zhang2021graphmi} & \checkmark                                  &                               &                             & 2021 & Attacks on GNNs                             \\
% Zheng et al. \cite{zheng2021efficient} &                                   & \checkmark                              &                          &  2021 & Private distributed framework for graph publication                              \\
% Zheng et al. \cite{zheng2021network} &   & \checkmark   &   &  2021 & Network Generation \\
% \end{tabular}
% }
% \caption{Summary of existing works on DP in graphs, ordered ascending by publication year and alphabetically within the same year. Ticks in the column \textbf{GNN} indicate whether the authors used GNNs in their work and ticks in columns \textbf{Edge-DP} and \textbf{Node-PD} specify whether the algorithms were applied under \textit{edge-level} or \textit{node-level} DP, respectively. Asterisk (*) denotes \textit{graph-level} DP and two asterisks (**) indicate that the DP notion is not clearly stated.}
% \label{tab:summary}
% \end{table*}



\begin{table*}[!ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccclll@{}}
\toprule
 & \textbf{Edge-DP} & \textbf{Node-DP} & \textbf{Graph-DP} & \textbf{LDP} & \textbf{Year} & \textbf{Reference}  &\textbf{Context} & \textbf{$\varepsilon$} \\
%  \toprule
% \midrule
 \midrule
  \multirow{45}{*}{\rotatebox[origin=c]{90}{\textbf{Graph Analysis}}} & \checkmark & \checkmark & & & 2007 & Nissim et al. \cite{nissim2007smooth}  & Estimation for spanning trees & -\\
  & \checkmark & & & & 2009 & Hay et al. \cite{hay2009accurate} & Graph degree estimation & $[0.01;1]$\\
  & \checkmark & & & & 2009 & Mir et al. \cite{mir2009differentially}  & Graph estimation  & -\\
  &  &  & & & 2011 & Gehrke et al.** \cite{gehrke2011towards} & Zero-knowledge statistics estimation & -\\
  & \checkmark & & & & 2011 & Machanavajjhala et al. \cite{machanavajjhala2011personalized}  & Privacy in social graphs & $[0.5;3]$\\
  & \checkmark & & & & 2011 & Sala et al. \cite{sala2011sharing} & Release of private graphs & $[0.1;100]$\\
  & \checkmark & & & & 2011 & Karwa et al. \cite{privateAnalysisGraph} & Private subgraph counting &$0.5$\\
  & \checkmark & & & & 2012 & Gupta et al. \cite{gupta2012iterative}  &  Synthetic data for graph cuts &-\\
  & \checkmark & & & & 2012 & Karwa et al. \cite{karwa2012differentially} &  Release of graph degree sequences &-\\
  & \checkmark & & & & 2012 & Mir et al. \cite{mir2012differentially} &  Private release of graph distribution &$0.2$\\
  & \checkmark & \checkmark &  & & 2013 & Blocki et al. \cite{blocki2013differentially} &  Restricted sensitivity for DP &-\\
  & & \checkmark & & & 2013 & Chen et al. \cite{chen2013recursive} &  Private graph database aggregation &$[0.1;0.5]$\\
  & & \checkmark & & & 2013 & Kasiviswanathan et al. \cite{kasiviswanathan2013analyzing} &  Private graph analysis &-\\
  & & & \checkmark & & 2013 & Shen et al. \cite{shen2013mining} &  Private graph pattern mining &$[0.1;1]$ \\
  & \checkmark & & & & 2013 & Wang et al. \cite{wang2013differential} & Private spectral graph analysis & $460$\\
  & \checkmark & & & & 2013 & Wang et al. \cite{wang2013preserving} & Private spectral graph analysis &-\\
  & \checkmark & & & & 2014 & Chen et al. \cite{chen2014correlated} & Correlated network data release & $[0.6;1]$\\
  & \checkmark & & & & 2014 & Lu et al. \cite{lu2014exponential} & Estimation of graph model parameters & $[0.1,1]$\\
  & & \checkmark & & & 2014 & Proserpio et al. \cite{proserpio2014calibrating} & Synthetic graph generation & $[0.01;10]$\\
  & \checkmark & \checkmark & \checkmark & & 2014 & Task et al. \cite{task2014should} &  Private social network analysis &-\\
  & & \checkmark & & & 2016 & Day et al. \cite{day2016publishing} &  Private graph distribution release &$[0.1;2]$\\
  & \checkmark & & & & 2016 & Jorgensen et al. \cite{jorgensen2016publishing} & Private attributed graph models &$[1;20]$\\
  & & \checkmark & & & 2016 & Raskhodnikova et al. \cite{raskhodnikova2016lipschitz} &  Private release of graph statistics & -\\
  & \checkmark & & & \checkmark & 2016 & Wang et al. \cite{wang2016using} &  Private aggregation of data & $[0;2]$\\
  & \checkmark & \checkmark & & \checkmark & 2017 & Qin et al. \cite{qin2017generating} & Private release of social graphs & $[0;7]$\\
  & \checkmark & \checkmark & & & 2017 & Zhu et al. \cite{zhu2017differential} &  Applications of differential privacy & - \\
  & \checkmark & \checkmark & & \checkmark & 2018 & Cormode et al. \cite{cormode2018privacy} & Private data release & - \\
  & & \checkmark & & & 2018 & Macwan et al. \cite{macwan2018node} & Private release of graph data & $0.5$\\
  & \checkmark & & & & 2019 & Arora et al. \cite{arora2019differentially}  &  Graph sparsification & -\\
  & & \checkmark & & & 2019 & Sealfon et al. \cite{ullman2019efficiently} & Estimation of graph statistics & -\\
  & & & & & 2019 & Sun et al. \cite{sun2019analyzing} & Subgraph statistics, decentralised DP & $[1;10]$ \\
  & & \checkmark & && 2019 & Yuxuan et al. \cite{yuxuan2019graph} &   Private histogram release &-\\
  & \checkmark & & & & 2020 & Chen et al. \cite{chen2020publishing} & Private synthetic data release & $[2;5]$\\
  & & \checkmark & & & 2020 & Liu et al. \cite{liu2020publishing} &  Node strength distribution  & $[0.1;2]$\\
  & & \checkmark & & & 2020 & Zhang et al. \cite{zhang2020community} &  Private social graph release & $[0.1;20]$\\
  & & \checkmark & & \checkmark & 2020 & Zhang et al. \cite{zhang2020differentially} &  Control-flow graph coverage analysis & $[2^{-5}; 2^5]$\\
  & & \checkmark & & & 2021 & Iftikhar et al. \cite{iftikhar2021dk} &  Private release of degree distribution & $[0.01;10]$\\
  & & \checkmark & & & 2021 & Fichtenberger et al. \cite{fichtenberger2021differentially} & Private dynamic graph algorithms & -\\
  & \checkmark & & & \checkmark & 2021 &  Imola et al. \cite{imola2021locally} &  Private sub-graph counting & $[0;2]$\\
  & & \checkmark & & & 2021 & Lan et al. \cite{lan2021sensitivity} & Private node strength histogram release & $[0.1;2]$ \\
  & & \checkmark & & & 2021 & Liu et al. \cite{liu2021graph} & Private degree histogram release  & $[0.1;2]$\\
  & & \checkmark & & & 2021 & Sealfon et al. \cite{sealfon2021efficiently} &  Private graph density estimation & -\\
  & \checkmark & \checkmark & & \checkmark & 2021 & Xia et al. \cite{xia2021dpgraph} & Benchmark platform for DP on graphs & - \\
  & \checkmark & & & \checkmark & 2021 & Zheng et al. \cite{zheng2021efficient}  & Private graph publication framework &-\\
  &\checkmark  & & & & 2021 & Zheng et al. \cite{zheng2021network} &  Network Generation & $[0.1;440]$\\
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{\textbf{GNNs}}} & \textbf{Edge-DP} & \textbf{Node-DP} & \textbf{Graph-DP} & \textbf{LDP} & \textbf{Year} &  \textbf{Reference} & \textbf{Context} & \textbf{$\varepsilon$}\\
% \cmidrule{2-8}
\midrule
     & & & & \checkmark & 2020 & Sajadmanesh et al.* \cite{sajadmanesh2020locally} & Locally private GNNs & $[0.01;3]$\\
     & & \checkmark & & & 2021 & Daigavane et al. \cite{daigavane2021node} & Node-level DP in GNNs & $[5;30]$\\
     &  & & & & 2021 & Igamberdiev et al.* \cite{igamberdiev2021privacy} & Private text classification & $[1;100]$\\  
     & & & & & 2021 & Olatunji et al.* \cite{olatunji2021releasing} & Private GNN and graph data release & $[1;40]$\\  
     & & & & & 2021 & Zhang et al.* \cite{zhang2021graphmi} & Attacks on GNNs &$[1;10]$ \\  
     & & & \checkmark && 2022 & Mueller et al. \cite{mueller2022differentially} & Graph-level DP for graph classification & $[0.5;20]$\\
\end{tabular}
}
\caption{Summary of existing works on DP on graphs, ordered ascending by publication year and alphabetically within the same year. The works are split into \textit{Graph Analysis} and \textit{GNNs}. Ticks in columns \textbf{Edge-DP}, \textbf{Node-DP}, and \textbf{Graph-DP} specify which notion of privacy was used. A tick in column \textit{LDP} indicates that the authors used local DP. The asterisks (*) indicates that the DP notion is not clearly stated. Two asterisks (**) indicate the utilisation of zero-knowledge privacy. The column $\varepsilon$ reports the privacy budget that was evaluated in the respective works.}
\label{tab:summary}
\end{table*}
